Are Machines Better at Complex Reasoning? Unveiling Human-Machine Inference Gaps in Entailment Verification

Making inferences in text comprehension to understand the meaning is essential in language processing. This work studies the entailment verification (EV) problem of multi-sentence premises that requires a system to make multiple inferences implicitly. Studying EV for such complex premises is important because modern NLP problems, such as detecting inconsistent model-generated rationales, require complex multi-hop reasoning. However, current textual inference datasets mostly contain short premises that only partially focus on these challenges. To address this, we compile an EV benchmark that includes datasets from three NLP domains (NLI, contextual QA, and rationales) containing multi-sentence premises. On benchmarking humans and LLMs, we find that LLMs are better than humans in multi-hop reasoning across extended contexts, while humans perform better in simple deductive reasoning tasks. We also finetune a Flan-T5 model for EV using two training objectives to obtain a strong open-source model that outperforms GPT-3.5 and rivals GPT-4. Finally, we use this model to filter out inconsistent model-generated rationales in self-consistency decoding, resulting in a 6% accuracy improvement on average across three MCQ datasets.

==> sections/figures.tex <==

%<*motivation>
% DO NOT REMOVE THESE TAGS
\begin{figure}[t]
	\centering
	\includegraphics[width=\columnwidth]{figures/example4.pdf}
	\caption{\small \textbf{Distinctions between human and LLM Inferences.} Examples of each reasoning type, along with the human and \gptfour{} prediction, are shown. A green box means the prediction matches the true label, and red otherwise. Humans are more consistent in simple deductive reasoning, whereas LLMs excel in complex, multi-step inferences over long contexts. Both humans and LLMs are comparable in instances with missing knowledge. Please refer to Section \ref{sec:human_alignment} for more details.}
	\label{fig:motivation}
	\vspace{-0.1cm}
\end{figure}
%</motivation>

%<*reasoningAnalysis1>
% DO NOT REMOVE THESE TAGS
\begin{figure*}[t]
	\centering
	\includegraphics[width=0.9\textwidth]{figures/reasoning_subplots.pdf}
	\caption{\small Analysis of different reasoning types involved in entailment verification for each dataset. \textbf{[Top]} Distribution of the reasoning types for each dataset studied. \textbf{[Bottom]} Macro-F1 performance comparison between humans and \gptfour{}. We fade out all bars with distribution percentage $\le$ 10\% since they are insignificant to draw meaningful conclusions. \textbf{Takeaways}: Humans are better at simple reasoning (\textbf{R1}) and commonsense reasoning (\textbf{R3}). \gptfour{} is superior at complex reasoning (\textbf{R2}) and entity-grounded reasoning (\textbf{R3} \anli{}). Trends for \textbf{R4} are mixed. Please refer to Appendix \ref{app:reasoning_analysis} for details.}
	\label{fig:reasoning_analysis1}
	\vspace{-0.4cm}
\end{figure*}
%</reasoningAnalysis1>

%<*reasoningAnalysis2>
% DO NOT REMOVE THESE TAGS
\begin{figure}[t]
	\centering
	\includegraphics[width=\columnwidth]{figures/reasoning_combined.pdf}
	\caption{\small Analysis of the different reasoning types involved in entailment verification. \textbf{[Top]} Distribution of the reasoning types aggregated across four datasets: \anli{}, \cosmosqa{}, \siqa{}, and \entailer{}. \textbf{[Bottom]} Performance comparisons between humans and \gptfour{}. \textbf{Takeaway}: \gptfour{} is better than humans at instances requiring complex reasoning, while humans are more consistent in simpler deductive reasoning tasks. Refer to Section \ref{sec:reasoning_type} for more details.}
	\label{fig:reasoning_analysis2}
	\vspace{-0.4cm}
\end{figure}
%</reasoningAnalysis2>

%<*cotFlowchart>
% DO NOT REMOVE THESE TAGS
\begin{figure*}[t]
	\centering
	\includegraphics[width=0.9\textwidth]{figures/cot_flowchart2.pdf}
	\caption{\small \textbf{Example of filtering CoT Rationales.} It consists of four steps: (1) CoT prompting, (2) Sampling multiple reasoning paths from the LLMs decoder, (3) Filtering out reasoning paths that don't support the model's prediction, (4) Aggregating the filtered reasoning paths to select the most consistent answer. The figure is inspired by self-consistency \cite{wang2023selfconsistency}. Note that we only filter \textit{inconsistent} rationales and not non-factual ones. Please refer to Section \ref{sec:filtering_cot} for more details.}
	\label{fig:cot_application}
	\vspace{-0.4cm}
\end{figure*}
%</cotFlowchart>

%<*cot>
% DO NOT REMOVE THESE TAGS
\begin{figure}[t]
	\centering
	\includegraphics[width=\columnwidth]{figures/cot_plot.pdf}
	\caption{\small Comparisons between self-consistency (SC) and Filtering + SC. We report the accuracy metric averaged across three MCQ datasets for four different LLMs. \textbf{Takeaway}: Filtering consistently improves performance over SC baseline, with more gains for weaker base models such as \ultwo{}. Please refer to Section \ref{sec:filtering_cot} for more details.}
	\label{fig:cot_comparison}
	\vspace{-0.4cm}
\end{figure}
%</cot>

%<*contextualQA>
% DO NOT REMOVE THESE TAGS
\begin{figure*}[t]
	\centering
	\includegraphics[width=0.9\textwidth]{figures/contextual_qa.pdf}
	\caption{\small \textbf{Example of Contextual QA data conversion.} For a given question and corresponding option, the QA-to-statement converter model generates a sentence combining the two. We use this as the hypothesis corresponding to that option. Please refer to Appendix \ref{app:dataset_statistics} for more details.}
	\label{fig:contextual_qa}
	\vspace{-0.4cm}
\end{figure*}
%</contextualQA>

%<*evalAnnotate>
% DO NOT REMOVE THESE TAGS
\begin{figure*}[t]
	\centering
	\includegraphics[width=0.97\textwidth]{figures/human_eval_format.pdf}
	\caption{\small \textbf{Human Evaluation Format.} We use this format to evaluate human performance on the Entailment Verification (EV) task. Please refer to Appendix \ref{app:human_ann_eval} for more details about the annotation procedure.}
	\label{fig:eval_annotate}
	\vspace{-0.3cm}
\end{figure*}
%</evalAnnotate>

%<*reasonAnnotate>
% DO NOT REMOVE THESE TAGS
\begin{figure*}[t]
	\centering
	\includegraphics[width=0.97\textwidth, height=0.97\textheight]{figures/reasoning_format.pdf}
	\caption{\small \textbf{Reasoning Type Annotation Format.} This format collects the reasoning type of sampled instances from each dataset. The detailed annotation procedure can be found in Append \ref{app:human_ann_reasoning}.}
	\label{fig:reason_annotate}
	\vspace{-0.3cm}
\end{figure*}
%</reasonAnnotate>

%<*k-selection>
% DO NOT REMOVE THESE TAGS
\begin{figure}[H]
	\centering
	\includegraphics[width=\columnwidth]{figures/k_selection.pdf}
	\caption{\small Results comparison among different $k$ values in CoT filtering application. $k=5$ is the best choice on average. For detailed analysis, please refer to Appendix \ref{app:top-k_analysis}.}
	\label{fig:k-selection}
	\vspace{-0.4cm}
\end{figure}
%</k-selection>

==> sections/tables.tex <==
%<*datasetComparisons>
% DO NOT REMOVE THESE TAGS
\begin{table*}[t]
	\centering
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{m{4.5cm}P{1cm}P{1cm}P{1cm}P{1cm}P{1cm}P{1.2cm}P{1cm}P{1cm}P{1cm}P{1cm}}
			\toprule
			\multirow{2}{*}{\textbf{\shortstack{Desirable\\Properties}}}  & \multicolumn{3}{c}{\textbf{{NLI}}} & \multicolumn{5}{c}{\textbf{{Contextual QA}}} & \multicolumn{2}{c}{\textbf{{Rationale}}} \\
			\cmidrule(r){2-4} \cmidrule(r){5-9} \cmidrule(r){10-11}
			& \wanli{} & \fever{} & \anli{} & \cosmosqa{} & \siqa{} & \dream{} & \boolq{} & \race{} & \entailer{} & \ecqa{} \\
			\midrule
			Multi-sentence premise & & \check & \check & \check & & \check & \check & \check & \check & \check \\
			Explanatory premise & & & & & & & & & \check & \check \\
			\midrule
			Entity-grounded knowledge & & \check & \check & & & & \check & & \check & \\
			Commonsense knowledge & & & & \check & \check & & & & & \check \\
			Localized knowledge & \check & & & \check & \check & \check & & \check & &\\
			\bottomrule
		\end{tabular}
	}
	\caption{Comparisons between different datasets used for evaluation. We compare on two broad categories: type of premise (multi-sentence and explanatory) and type of knowledge tested (entity-grounded, commonsense, and localized). Please refer to Section \ref{sec:datasets} for more details.}
	\label{tab:dataset_comparisons}
	\vspace{-0.1cm}
\end{table*}
%</datasetComparisons>

%<*knowledgeExamples>
% DO NOT REMOVE THESE TAGS
\begin{table}[t]
	\scriptsize
	\centering
	\resizebox{0.95\columnwidth}{!}{%
		\begin{tabular}{m{2cm}m{3.5cm}}
			\toprule
			\textbf{Knowledge} & \textbf{Examples} \\
			\midrule
			Entity-grounded & Barack Obama is born in USA.; Electrical energy is used by plants for making food. \\
			Commonsense & If you are hurting, you might cry.; If you steal something, you can get in trouble.\\
			Localized & The policeman helps her find her daughter.; Dan is 72 years old currently.\\
			\bottomrule
		\end{tabular}
	}
	\caption{Examples of different categories of knowledge. Please refer to Section \ref{sec:datasets} for more details.}
	\label{tab:knowledge_examples}
	\vspace{-0.4cm}
\end{table}
%</knowledgeExamples>

%<*humanResults>
% DO NOT REMOVE THESE TAGS
\begin{table*}[t]
	\centering
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{m{2.6cm}P{1cm}P{1cm}P{1cm}P{1cm}P{1cm}P{1.2cm}P{1cm}P{1cm}P{1cm}P{1cm}P{1cm}}
			\toprule
			\multirow{2}{*}{\textbf{Model}}  & \multicolumn{3}{c}{\textbf{{NLI}}} & \multicolumn{5}{c}{\textbf{{Contextual QA}}} & \multicolumn{2}{c}{\textbf{{Rationale}}} & \multirow{2}{*}{\textbf{\shortstack{Avg}}} \\
			\cmidrule(r){2-4} \cmidrule(r){5-9} \cmidrule(r){10-11}
			& \wanli{} & \fever{} & \anli{} & \cosmosqa{} & \siqa{} & \dream{} & \boolq{} & \race{} & \entailer{} & \ecqa{} \\
			\midrule
			\roberta{} & \textbf{0.81} & \textbf{0.92} & 0.67 & 0.46 & 0.45 & 0.63 & 0.71 & 0.41 & 0.87 & 0.37 & 0.63 \\
			\entailermx{} & 0.68 & 0.75 & 0.59 & 0.71 & 0.56 & 0.67 & 0.81 & 0.49 & \textbf{0.91} & \textbf{0.49} & 0.67 \\
			\midrule
			\flantxxl{} & 0.71 & 0.79 & 0.68 & 0.66 & 0.55 & 0.79 & \textbf{0.86} & 0.60 & 0.88 & \textbf{0.49} & 0.70 \\
			\gptthree{} & 0.76 & 0.81 & 0.62 & 0.67 & 0.59 & 0.79 & 0.76 & 0.52 & 0.76 & 0.48 & 0.68 \\
			\gptfour{} & 0.79 & 0.86 & \textbf{0.79} & \textbf{0.76} & 0.61 & \textbf{0.90} & 0.84 & \textbf{0.68} & 0.80 & 0.48 & \textbf{0.75} \\
			\midrule
			\multirow{2}{*}{Human} & 0.74 & 0.88 & 0.67 & 0.63 & \textbf{0.74} & 0.87 & 0.77 & 0.61 & \textbf{0.91} & 0.48 & 0.73 \\
			& \textit{(0.78)} & \textit{(0.75)} & \textit{(0.62)} & \textit{(0.51)} & \textit{(0.54)} & \textit{(0.68)} & \textit{(0.67)} & \textit{(0.57)} & \textit{(0.82)} & \textit{(0.85)} & \textit{(0.68)} \\
			\midrule
			Human $-$ \gptfour{} & -0.05 & 0.02 & -0.12 & -0.13 & 0.13 & -0.03 & -0.07 & -0.07 & 0.11 & 0.00 & -0.02 \\
			\bottomrule
		\end{tabular}
	}
	\caption{Comparisons between human and baseline LLMs on 100 sampled instances from each dataset. We report the macro-F1 score and highlight the best results in bold. For the human baseline, we report the annotation agreements in parenthesis. \textbf{Takeaways}: Task-finetuned models perform well on specific dataset categories seen during finetuning, but instruction-finetuned models generalize better on average. \gptfour{} is the best-performing LLM. It outperforms humans on \anli{} and \cosmosqa{} that require complex, multi-step reasoning. In contrast, humans are better on \siqa{} and \entailer{} that require simple deductive reasoning. Please refer to Section \ref{sec:human_performance} for more analysis.}
	\label{tab:human_results}
	\vspace{-0.4cm}
\end{table*}
%</humanResults>


%<*finetuneResults>
% DO NOT REMOVE THESE TAGS
\begin{table*}[t]
	\centering
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{m{4cm}P{1cm}P{1cm}P{1cm}P{1cm}P{1cm}P{1.2cm}P{1cm}P{1cm}P{1cm}P{1cm}P{1cm}P{1cm}P{1cm}}
			\toprule
			\multirow{2}{*}{\textbf{Model}}  & \multicolumn{3}{c}{\textbf{{NLI}}} & \multicolumn{5}{c}{\textbf{{Contextual QA}}} & \multicolumn{2}{c}{\textbf{{Rationale}}} & \multirow{2}{*}{\textbf{\shortstack{Avg}}} & \multirow{2}{*}{\textbf{\shortstack{Seen\\Avg}}} & \multirow{2}{*}{\textbf{\shortstack{Unseen\\Avg}}} \\
			\cmidrule(r){2-4} \cmidrule(r){5-9} \cmidrule(r){10-11}
			& \wanli{} & \fever{} & \anli{}$^\dagger$ & \cosmosqa{} & \siqa{} & \dream{} & \boolq{} & \race{}$^\dagger$ & \entailer{} & \ecqa{}$^\dagger$ \\
			\midrule
			\gptfour{} & \textbf{0.73} & \textbf{0.88} & \textbf{0.86} & 0.79 & 0.69 & \textbf{0.92} & \textbf{0.86} & \textbf{0.85} & \textbf{0.86} & 0.48 & 0.79 & - & - \\
			\gptthree{} & 0.70 & 0.83 & 0.69 & 0.70 & 0.67 & 0.81 & 0.78 & 0.69 & 0.82 & 0.48 & 0.72 & - & - \\
			\flantxxl{} & 0.63 & 0.81 & 0.73 & 0.59 & 0.67 & 0.80 & 0.85 & 0.70 & 0.83 & \textbf{0.50} & 0.71 & - & - \\
			\midrule
			\ourclass & 0.71 & 0.86 & 0.79 & 0.66 & 0.72 & 0.88 & 0.85 & \textbf{0.85} & 0.85 & 0.49 & 0.77 & 0.71 & 0.79 \\
			\ourrank & 0.69 & 0.85 & 0.77 & \textbf{0.83} & \textbf{0.74} & 0.89 & 0.85 & \textbf{0.85} & \textbf{0.86} & 0.48 & 0.78 & 0.70 & 0.82 \\
			\bottomrule
		\end{tabular}
	}
	\caption{Comparison of classification and ranking-based \flantxxl{} finetuning with baseline LLMs on the complete evaluation benchmark. We report the macro-F1 for all datasets. $^\dagger$: Dataset is used in fine-tuning, and the average is reported in the ``Seen Avg'' column. Other datasets are zero-shot evaluated, and the average is reported in the ``Unseen Avg'' column. \textbf{Takeaways}: Ranking objective is better than classification on contextual QA datasets. \ourrank{} outperforms \flantxxl{} and \gptthree{}, and performs comparably to \gptfour{}. Please refer to Section \ref{sec:finetuning_results} for more details.}
	\label{tab:finetune_results}
	\vspace{-0.4cm}
\end{table*}
%</finetuneResults>


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Appendix Tables
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%<*cotResults>
% DO NOT REMOVE THESE TAGS
\begin{table*}[t]
	\centering
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{m{9cm}P{2cm}P{2cm}P{2cm}P{2cm}}
			\toprule
			\textbf{Method} & \csqa{} & \arce{} & \arcc{} & Average \\
			\midrule
			UL2 + SC & 55.77 & 70.33 & 49.57 & 58.56 \\
			UL2 + Filter (\flantxxl{}) + SC & 62.49	& 74.50	& 55.72 & 64.24 \\
			UL2 + Filter (\ourrank{}) + SC & 63.80 & 77.24 & 60.08 & 67.04 \\
			\midrule
			Codex-001 + SC & 54.80 & 71.70 & 52.20 & 59.57 \\
			Codex-001 + Filter (\flantxxl{}) + SC & 65.44 & 73.57 & 54.27 & 64.43 \\
			Codex-001 + Filter (\ourrank{}) + SC & 68.39 & 78.16 & 59.51 & 68.69 \\
			\midrule
			LaMDA-137B + SC & 62.90 & 78.90 & 59.90 & 67.23 \\
			LaMDA-137B + Filter (\flantxxl{}) + SC & 71.17 & 80.89 & 63.65 & 71.90 \\
			LaMDA-137B + Filter (\ourrank{}) + SC & 72.15 & 82.95 & 67.32 & 74.14 \\
			\midrule
			ChatGPT + SC & 78.40 & 96.30 & 87.20 & 87.30 \\
			ChatGPT + Filter (\flantxxl{}) + SC & 81.86 & 96.52 & 88.32 & 88.90 \\
			ChatGPT + Filter (\ourrank{}) + SC & 81.88 & 96.57 & 88.63 & 89.03 \\
			\bottomrule
		\end{tabular}
	}
	\caption{Comparison of Chain-of-Thought filtering performance. We consider four self-consistency baselines. For each baseline, we experiment with both \flantxxl{} and \ourrank{} to filter out inconsistent rationals. \textbf{Takeaway}: Our fintuning strategy brings notable improvements when compared to both baseline and \flantxxl{} filtering model. For more details and analysis, please check Appendix \ref{app:cot_filtering}.}
	\label{tab:cot_results}
\end{table*}
%</cotResults>



%<*filterExamples>
% DO NOT REMOVE THESE TAGS
\begin{table*}[t]
	\centering
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{p{6cm}p{10cm}P{1cm}}
			\toprule
			\textbf{Question \& Options} &\textbf{(Rationale, Prediction)} & \textbf{Kept} \\
			\midrule
			\multirow{5}{6cm}{\textbf{[ARC\_easy]} \newline Cells need nutrients for energy. Which system is responsible for breaking down food to provide cellular energy? \newline \textbf{(A)} digestive \newline \textbf{(B)} excretory \newline \textbf{(C)} circulatory \newline \textbf{(D)} respiratory} & (Digestive system takes in food, breaks down food, and takes away the unusable parts of the food using the excretory system., \textbf{B}) & \check \\
			\cmidrule(r){2-3}
			& (Circulatory system is responsible for eliminating waste from the body. Circulatory system is also responsible for breaking down food into nutrients that the cells can use., \textbf{C}) & \check \\
			\cmidrule(r){2-3}
			& (Cellular energy is provided by the chemical breakdown of food., \textbf{C}) & \cross \\
			\cmidrule(r){2-3}
			& (In the mouth, food is broken down and absorbed into the circulatory system., \textbf{D}) & \cross \\
			\cmidrule(r){2-3}
			& (Since the digestive system breaks down food to provide cellular energy., \textbf{B}) & \cross \\
			\midrule
			
			\multirow{5}{6cm}{\textbf{[CSQA]} \newline A human wants to submerge himself in water, what should he use? \newline \textbf{(A)} whirlpool bath \newline \textbf{(B)} coffee cup \newline \textbf{(C)} cup \newline \textbf{(D)} soft drink \newline \textbf{(E)} puddle} & (The answer should be the thing that will help the human submerge himself in water. Of the above choices, only whirlpool baths can help the human submerge himself in water., \textbf{A}) & \check \\
			\cmidrule(r){2-3}
			& (The answer should be an item that allows the human to fully submerge himself. Of the above choices, only a whirlpool bath allows the human to fully submerge himself., \textbf{A}) & \check \\
			\cmidrule(r){2-3}
			& (The answer should be something that can perform the submerging function. Of the above choices, only the soft drink can float., \textbf{D}) & \cross \\
			\cmidrule(r){2-3}
			& (The answer must be something that a human would use. Of the above choices, the only thing a human would use is a soft drink., \textbf{D}) & \cross \\
			\cmidrule(r){2-3}
			& (The answer must be something that is liquid. Of the above choices, only a cup of water is liquid., \textbf{C}) & \cross \\
			\midrule
			
			\multirow{7}{6cm}{\textbf{[ARC\_challenge]} \newline In pea plants, the trait for round seeds is dominant over the trait for wrinkled seeds. If a pure dominant plant with round seeds is crossed with a plant with wrinkled seeds, what can be predicted about the offspring plants? \newline \textbf{(A)} They will always produce round seeds. \newline \textbf{(B)} They will only produce wrinkled seeds. \newline \textbf{(C)} Each offspring plant will have some round and some wrinkled seeds. \newline \textbf{(D)} Unless the plant with wrinkled seeds was pure recessive, no prediction can be made.} & (The offspring plants will only produce round seeds as the round seed trait is dominant over the wrinkled seed trait., \textbf{A}) & \check \\
			\cmidrule(r){2-3}
			& (If plant with round seeds is crossed with plant with wrinkle seeds, the dominant trait will be passed down to the offspring; so each offspring plant will have round seeds., \textbf{A}) & \check \\
			\cmidrule(r){2-3}
			& (If a pure dominant plant with round seeds is crossed with a plant with wrinkled seeds, the offspring plant will produce round seeds., \textbf{C}) & \cross \\
			\cmidrule(r){2-3}
			& (Just like the traits in humans, there is no dominant trait for a particular characteristic., \textbf{C}) & \cross \\
			\cmidrule(r){2-3}
			& (The recessive trait is the one that causes the plant to produce round seeds. So option Unless the plant with wrinkled seeds was pure recessive, no prediction can be made., \textbf{D}) & \cross \\
			\\
			\\
			\bottomrule
		\end{tabular}%
	}
	\caption{CoT filtering examples from three MCQ datasets. Each example contains two outputs that are kept and three outputs that are filtered out in the entailment verification pipeline. Please refer to Appendix \ref{app:cot_examples} for more details.}
	\label{tab:filter_examples}
\end{table*}
%</filterExamples>

%<*dataStatistic>
% DO NOT REMOVE THESE TAGS
\begin{table*}[t]
	\centering
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{m{2.3cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.2cm}}
			\toprule
			\multirow{2}{*}{\textbf{\shortstack[l]{Dataset\\ Statistics}}}  & \multicolumn{3}{c}{\textbf{{NLI}}} & \multicolumn{5}{c}{\textbf{{Contextual QA}}} & \multicolumn{2}{c}{\textbf{{Rationale}}} \\
			\cmidrule(r){2-4} \cmidrule(r){5-9} \cmidrule(r){10-11}
			& \wanli{} & \fever{} & \anli{} & \cosmosqa{} & \siqa{} & \dream{} & \boolq{} & \race{} & \entailer{} & \ecqa{} \\
			\midrule
			Train & 102,885 & 208,346 & 162,865 & 77,468 & 100,212 & 18,348 & 18,854 & 341,412 & - & 7,598 \\
            Dev & - & 19,998 & 3,200 & 8,970 & 5,859 & 6,120 & 6,540 & 18,944 & 7,849 & 1,090 \\
            Test & 5,000 & - & 3,200 & - & - & 6,123 & - & 19,172 & - & 2,194 \\
			\bottomrule
		\end{tabular}
	}
	\caption{The number of examples in train/dev/test splits for different datasets. Some datasets do not have certain splits, and those statistics are left blank. For each dataset in our benchmark, we use the test split if available; otherwise, we use the dev split. Please refer to Appendix \ref{app:dataset_statistics} for more details about each dataset.}
	\label{tab:dataset_statistics}
\end{table*}
%</dataStatistic>

%<*promptSensitivity>
% DO NOT REMOVE THESE TAGS
\begin{table*}[t]
	\centering
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{m{16.5cm} | P{1cm}}
			\toprule
			\textbf{Prompt} & \textbf{Avg} \\
			\midrule
            Premise: \{premise\}\textbackslash n Hypothesis: \{hypothesis\}\textbackslash n Given the premise, is the hypothesis correct?\textbackslash n Answer: & 0.71 \\
            Premise: \{premise\}\textbackslash n Hypothesis: \{hypothesis\}\textbackslash n Given the premise, is the hypothesis supported?\textbackslash n Answer: & 0.70 \\
            Premise: \{premise\}\textbackslash n Hypothesis: \{hypothesis\}\textbackslash n Based on the premise, is the hypothesis correct?\textbackslash n Answer: & 0.71 \\
            Premise: \{premise\}\textbackslash n Hypothesis: \{hypothesis\}\textbackslash n Does the premise support the hypothesis?\textbackslash n Answer: & 0.69 \\
            Given the premise \{premise\}, is the hypothesis \{hypothesis\} supported?\textbackslash n Answer: & 0.70 \\
            We are given the premise: \{premise\}. Can we conclude the hypothesis: \{hypothesis\}?\textbackslash n Answer: & 0.72 \\
			\bottomrule
		\end{tabular}
	}
	\caption{Comparison of averaged results between different prompt formats used for \flantxxl{} evaluation. \textbf{Takeaway}: The model is robust to variations in the prompt and generates consistent results. Please refer to Appendix \ref{app:instruction_finetuned} for more details.}
	\label{tab:prompt_sensitivity}
\end{table*}
%</promptSensitivity>

%<*reasoningExamples>
% DO NOT REMOVE THESE TAGS
\begin{table*}[t]
	\centering
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{p{1.5cm}p{13cm}P{1cm}P{1cm}P{1cm}}
			\toprule
			\textbf{Type} &\textbf{Example} & \textbf{Entails} & \textbf{Human} & \textbf{GPT4} \\
			\midrule
			\multirow{3}{*}{\textbf{[R1]}} & \textbf{Premise}: Seoul Train is a 2004 documentary film that deals with the dangerous journeys of North Korean defectors fleeing through or to China. These journeys are both dangerous and daring, since if caught, they face forced repatriation, torture, and possible execution. \newline \textbf{Hypothesis}: Seoul Train was filmed in 2002 to depict the dangerous journey of North Korea. & No & \cross & \check \\
			\cmidrule(r){2-5}
			& \textbf{Premise}: My family history goes back a long way. My ancestors on my mothers side were a mix of English and Scandinavian Mormon converts that came to Utah in the 19th century. My father side is an unknown. \newline \textbf{Hypothesis}: It might be true that your family history has a short history. & No & \check & \check \\
			\cmidrule(r){2-5}
			& \textbf{Premise}: An iron oxide can be made from oxygen and rust. Oxygen and rust are gases at room temperature. \newline \textbf{Hypothesis}: An iron oxide can be made from two elements that are gases at room temperature. & Yes & \check & \cross \\
			\midrule
			
			\multirow{3}{*}{\textbf{[R2]}} & \textbf{Premise}: How to make deep fried watermelon. Cut the watermelon in half, down its length. Then cut each half in half, again cutting down the length. Place the four wedges on a board for cutting. \newline \textbf{Hypothesis}: To deep fry a watermelon, it should be cut into 6 pieces. & No & \cross & \check \\
			\cmidrule(r){2-5}
			& \textbf{Premise}: The freshwater mussels used to live in the place where the mountain range is located. A freshwater mussel is a kind of water animal that lives in freshwater. \newline \textbf{Hypothesis}: The mountain range used to be covered by freshwater. & Yes & \check & \cross \\
			\cmidrule(r){2-5}
			& \textbf{Premise}: De Baandert was a multi-use stadium in Sittard-Geleen, Netherlands. It was used mostly for football matches and hosted the home matches of Fortuna Sittard. The stadium was able to hold 22,000 people. It was closed in 1999 when Fortuna Sittard Stadion opened. \newline \textbf{Hypothesis}: 22,000 people go to football matches at De Baandert. & No & \cross & \check \\
			\midrule
			
			\multirow{3}{*}{\textbf{[R3]}} & \textbf{Premise}: Sasha spent Austin's money trying to win a prize even when the odds were stacked against her. \newline \textbf{Hypothesis}: Austin will want to pull out more money next. & No & \cross & \check \\
			\cmidrule(r){2-5}
			& \textbf{Premise}: George Dayton (born 1827, died 1938) lived in Union Township in what is now Rutherford, New Jersey, and represented Bergen County in the New Jersey Senate from 1875 to 1877. Dayton moved to Closter, New Jersey, in 1890 and became the clerk of Harrington Township, New Jersey. \newline \textbf{Hypothesis}: George Dayton lived in New Jersey his entire life. & No & \cross & \cross \\
			\cmidrule(r){2-5}
			& \textbf{Premise}: We fought aliens on Mars for Mars Bars, which gave us superspeed. We didn't stop at Jupiter, coz that would have made us "stupider". Pluto was very chilly, so we ate it. Ahem, chille that is. \newline \textbf{Hypothesis}: This person will attempt to make a fun rhyme with the names of the other six planets. & Yes & \check & \cross \\
			\midrule
			
			\multirow{3}{*}{\textbf{[R4]}} & \textbf{Premise}: Robin put their hand on Addison's wrist to keep Addison from shaking uncontrollably. \newline \textbf{Hypothesis}: Addison will want to do good next. & No & \cross & \check \\
			\cmidrule(r){2-5}
			& \textbf{Premise}: Terry Pratchett's Going Postal is a two-part television film adaptation of "Going Postal" by Terry Pratchett, adapted by Richard Kurti and Bev Doyle and produced by The Mob, which was first broadcast on Sky1, and in high definition on Sky1 HD, at the end of May 2010. \newline \textbf{Hypothesis}: Terry Pratchett's Going Postal adaptation for television is faithful to the original novel. & No & \cross & \check \\
			\cmidrule(r){2-5}
			& \textbf{Premise}: Co-producing the film is Happy Madison, the company owned by Sandler, who has been a compatriot of Schneider's since they met early in their careers, as mutually struggling stand-up comedians in Los Angeles. \newline \textbf{Hypothesis}: Comedians in Los Angeles struggle. & No & \check & \cross \\
			\bottomrule			
		\end{tabular}%
	}
	\caption{Comparison between the performance of humans and \gptfour{} on examples from four reasoning types. Each example includes the golden label from the dataset and shows if human/\gptfour{} makes the correct decision. The definition of those reasoning types and detailed analysis can be found in Section \ref{sec:reasoning_type} and Appendix \ref{app:reasoning_examples}.}
	\label{tab:reasoning_examples}
\end{table*}
%</reasoningExamples>

%<*fewshotResults>
% DO NOT REMOVE THESE TAGS
\begin{table*}[t]
	\centering
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{m{5.5cm}P{1cm}P{1cm}P{1cm}P{1cm}P{1cm}P{1.2cm}P{1cm}P{1cm}P{1cm}P{1cm}P{1cm}P{1cm}P{1cm}}
			\toprule
			\multirow{2}{*}{\textbf{Model}}  & \multicolumn{3}{c}{\textbf{{NLI}}} & \multicolumn{5}{c}{\textbf{{Contextual QA}}} & \multicolumn{2}{c}{\textbf{{Rationale}}} & \multirow{2}{*}{\textbf{\shortstack{Avg}}} \\
			\cmidrule(r){2-4} \cmidrule(r){5-9} \cmidrule(r){10-11}
			& \wanli{} & \fever{} & \anli{} & \cosmosqa{} & \siqa{} & \dream{} & \boolq{} & \race{} & \entailer{} & \ecqa{} \\
			\midrule
            \gptfour{} & 0.73 & 0.88 & 0.86 & 0.79 & 0.69 & 0.92 & 0.86 & 0.85 & 0.86 & 0.48 & 0.79 \\
            \gptfour{} + \textit{few-shot} & 0.75 & 0.87 & 0.84 & 0.75 & 0.62 & 0.91 & 0.86 & 0.81 & 0.83 & 0.48 & 0.77 \\
            \midrule
			\flantxxl{} & 0.63 & 0.81 & 0.73 & 0.59 & 0.67 & 0.80 & 0.85 & 0.70 & 0.83 & 0.50 & 0.71 \\
            \flantxxl{} + \textit{few-shot} & 0.67 & 0.84 & 0.77 & 0.66 & 0.71 & 0.84 & 0.84 & 0.74 & 0.85 & 0.49 & 0.74 \\
            \midrule
			\ourrank & 0.69 & 0.85 & 0.77 & 0.83 & 0.74 & 0.89 & 0.85 & 0.85 & 0.86 & 0.48 & 0.78 \\
            \ourrank{} + \textit{few-shot} & 0.69 & 0.86 & 0.79 & 0.77 & 0.74 & 0.89 & 0.84 & 0.85 & 0.86 & 0.48 & 0.78 \\
			\bottomrule
		\end{tabular}
	}
	\caption{Comparison of performance between base models and models with few-shot setting. \textbf{Takeaway}: For \flantxxl{}, few-shot prompting boosts the performance, while it is not beneficial for the other two models. Please refer to Appendix \ref{app:instruction_finetuned} for more analysis.}
	\label{tab:fewshot_results}
\end{table*}
%</fewshotResults>

%<*majorityResults>
% DO NOT REMOVE THESE TAGS
\begin{table}[t]
	\centering
	\resizebox{0.7\columnwidth}{!}{%
		\begin{tabular}{m{2.7cm}P{3.5cm}}
			\toprule
			\textbf{Dataset} & \textbf{Majority Prediction} \\
			\midrule
            \wanli{} & 0.39 \\
            \fever{} & 0.40 \\
            \anli{} & 0.40 \\
            \midrule
            \cosmosqa{} & 0.41 \\
            \siqa{} & 0.40 \\
            \dream{} & 0.40 \\
            \boolq{} & 0.35 \\
            \race{} & 0.43 \\
            \midrule
            \entailer{} & 0.43 \\
            \ecqa{} & 1.00 \\
			\bottomrule
		\end{tabular}
	}
	\caption{The macro-F1 score of majority label (most frequent label) prediction for different datasets. For reference, the score of a well-balanced dataset is 0.67. Those figures indicate that the label imbalance issue exists in the datasets we evaluate. More details are presented in Appendix \ref{app:majority_baseline}.}
	\label{tab:majority_results}
\end{table}
%</majorityResults>

%<*contextualExamples>
% DO NOT REMOVE THESE TAGS
\begin{table*}[t]
	\centering
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{p{8cm}p{8cm}}
			\toprule
			\textbf{Question \& Options} &\textbf{Corresponding Hypothesis of Option} \\
			\midrule
            \multirow{7}{7.7cm}{Alex told a very scary ghost store to the campers around the campfire. What will Skylar want to do next? \newline \newline \textbf{(A) run screaming} \newline (B) laugh it all \newline (C) cry}
            & \\
            & \\
            & \\
            & \\
            & \textbf{Skylar will want to run screaming next.} \\
            & Skylar will want to laugh it all next. \\
            & Skylar will want to cry next. \\
			\midrule
			\multirow{8}{7.7cm}{After finalizing the plans with the architect and the contractors, Austin built Quinn's house last week. How would Quinn feel as a result? \newline \newline (A) intrigued by the building of the house \newline \newline \textbf{(B) grateful for the hard work that was done} \newline \newline (C) curious about why the house was built}
            & \\
            & \\
            & \\
            & \\
            & Quinn would feel intrigued by the building of the house as a result. \\
			& \textbf{Quinn would feel grateful for the hard work that was done as a result.} \\
            & Quinn would feel curious about why the house was built as a result. \\
			\bottomrule
		\end{tabular}%
	}
	\caption{Examples from Contextual QA datasets with a debatable hypothesis. The correct answers are marked. More analysis can be found in Appendix \ref{app:debatable_example}.}
	\label{tab:contextual_examples}
\end{table*}
%</contextualExamples>
